Singular perturbation results for linear partial differential-algebraic equations of hyperbolic type

We consider constrained partial differential equations of hyperbolic type with a small parameter $\varepsilon>0$, which turn parabolic in the limit case, i.e., for $\varepsilon=0$. The well-posedness of the resulting systems is discussed and the corresponding solutions are compared in terms of the parameter $\varepsilon$. For the analysis, we consider the system equations as partial differential-algebraic equation based on the variational formulation of the problem. For a particular choice of the initial data, we reach first- and second-order estimates. For general initial data, lower-order estimates are proven and their optimality is shown numerically.

==> def.tex <==
%% specific things for hyperbolic pipes
%
%%% various bar sizes
\makeatletter
\newsavebox\myboxA
\newsavebox\myboxB
\newlength\mylenA
%
\newcommand*\xoverline[2][0.75]{%
	\sbox{\myboxA}{$\m@th#2$}%
	\setbox\myboxB\null% Phantom box
	\ht\myboxB=\ht\myboxA%
	\dp\myboxB=\dp\myboxA%
	\wd\myboxB=#1\wd\myboxA% Scale phantom
	\sbox\myboxB{$\m@th\overline{\copy\myboxB}$}%  Overlined phantom
	\setlength\mylenA{\the\wd\myboxA}%   calc width diff
	\addtolength\mylenA{-\the\wd\myboxB}%
	\ifdim\wd\myboxB<\wd\myboxA%
	\rlap{\hskip 0.5\mylenA\usebox\myboxB}{\usebox\myboxA}%
	\else
	\hskip -0.5\mylenA\rlap{\usebox\myboxA}{\hskip 0.5\mylenA\usebox\myboxB}%
\fi}
%
%%% right-hand sides %%%
\def\f{g}
\def\g{f}
\def\h{h} 					% boundary conditions --> ehemals \Ge
%\def\r{r} 					%					  --> ehemals \Gi
%
%%% constraint operators %%%
\def\Ci{{\C}}   			% point evaluation - interior/outflow
\def\Ce{{\B}}   			% point evaluation - inflow
\def\Di{{\calR}}   			% linear comb.     - interior/outflow
\def\De{{\calR_\text{in}}}  % linear comb.     - inflow
%\def\Ded{{\calR^*_\text{in}}} % dual operator 
%
%%% graph stuff %%%
\def\Vin{{\V_\text{pot}}}			% vertives with inflow (bc for p)
\def\Vout{ \V \setminus \Vin }		% vertives - interior or outflow
%
\def\Nout{{M}}		% # vertices - coupling/outflow
\def\Nin{{N}}		% # vertices - inflow

% test functions
\def\u{w}

% -+ since \mp is redefined 
\newcommand{\minusplus}{\mp}

\newcommand*{\potL}[1][0]{p^{\vee\hspace{-0.31em}\wedge}_{#1,\tau}}
\newcommand*{\potC}[1][0]{p^{\overline{~} \hspace{-0.06em} \underline{~} }_{#1,\tau}}
\newcommand*{\phtL}{{\hat p}^{\vee\hspace{-0.31em}\wedge}_{\tau\phantom{|}}}
\newcommand*{\phtC}{{\hat p}^{\overline{~} \hspace{-0.06em} \underline{~} }_{\tau\phantom{|}}}
%
\newcommand*{\potPol}[3]{\Pi_{#2} p_{#1 #3}}
\newcommand*{\phtPol}[1]{\Pi_{#1} {\hat p}_{\tau}}
%
\newcommand*{\motC}[1][0]{m^{\overline{~} \hspace{-0.06em} \underline{~} }_{#1,\tau}}
\newcommand*{\mhtC}{{\hat m}^{\overline{~} \hspace{-0.06em} \underline{~} }_{\tau\phantom{|}}}
\newcommand*{\muotC}[1][0]{\mu^{\overline{~} \hspace{-0.06em} \underline{~} }_{#1,\tau}}

%
\newcommand*{\motPol}[3]{\Pi_{#2} m_{#1 #3}}
\newcommand*{\mhtPol}[1]{\Pi_{#1} {\hat m}_{\tau}}
%

% für den seltsamen Startwert
\def\mstar{\mathfrak h}
\def\pstar{\mathfrak p}
\def\pstarII{\widetilde{\mathfrak p}}


% splitting solutions
\def\ph{p_\text{h}}
\def\pp{p_\text{p}}
\def\mh{m_\text{h}}
\def\mp{m_\text{p}} 

% amax, dmin, dmax
\def\aM{a_\text{max}}
\def\dm{d_\text{min}}
\def\dM{d_\text{max}}

%
\renewcommand{\div}{\operatorname{div}} 
\newcommand{\Md}{M_d}
\newcommand{\Ma}{M_a}
%
\def\N{\mathbb{N}}
\def\I{\mathbb{I}}
\def\R{\mathbb{R}}
%
\def\A{\mathcal{A}}
\def\B{\mathcal{B}} 
\def\C{\mathcal{C}}
\def\D{\mathcal{D}}
\def\E{\mathcal{E}}
\def\bE{\bar{\mathcal{E}}}
\def\F{\mathcal{F}}
\def\G{\mathcal{G}}
\def\cH{\mathcal{H}}
\def\calH{\mathcal{H}}
\def\cHker{\cH_{\ker}}
\def\calI{\mathcal{I}}
\def\K{\mathcal{K}}
\def\calK{\mathcal{K}}
\def\calL{\mathcal{L}}
\def\M{\mathcal{M}}
\def\calM{\mathcal{M}}
\def\O{\mathcal{O}}
\def\P{\mathcal{P}}
\def\Pker{\P_{\ker}}
\def\Q{\mathit{\Lambda}}  %{\mathcal{Q}}
\def\calR{\mathcal{R}}
\def\S{\mathcal{S}}
\def\T{\mathcal{T}}
\def\V{\mathcal{V}}
\def\X{\mathcal{X}}

\def\wlap{\mathcal{L}}
\def\cLap{c_\mathcal{L}}
%
\def\eps{\varepsilon}

%%%% Colors
\definecolor{blau}{RGB}{0, 51, 255}
\definecolor{hellblau}{RGB}{153, 204, 255}
\definecolor{hellrot}{RGB}{255, 0, 0}
\definecolor{firebrick}{RGB}{176, 34, 34} 
\definecolor{deep_pink}{RGB}{255, 20, 147} 
\definecolor{sky_blue}{RGB}{74, 112, 139}
\definecolor{slate_blue}{RGB}{71, 60, 139}
\definecolor{chartreuse}{RGB}{118, 238, 0}
\definecolor{chartreuseL}{RGB}{228, 255, 150}
\definecolor{light_blue}{RGB}{178, 223, 238}
\definecolor{dodge_blue}{RGB}{17, 78, 138}
\definecolor{code_backg}{RGB}{238, 216, 174}
%
\definecolor{myBlue1}{RGB}{101,149,239}  % cornflowerblue
\definecolor{myBlue2}{RGB}{113,104,238} % medium slate blue	
\definecolor{myBlue3}{RGB}{30,144,255} % dodger blue
\definecolor{myGreen1}{RGB}{154,204,50} % yellow green
\definecolor{myGreen2}{RGB}{69,169,0} % chatreuse
\definecolor{myGreen3}{RGB}{154,205,50} % olive Drap
\definecolor{myGreen4}{RGB}{105,139,34} % olive Drap2
\definecolor{myRed1}{RGB}{210,105,30} % chocolate
\definecolor{myRed2}{RGB}{165,42,42} % brown
\definecolor{myRed3}{RGB}{139,26,26} % firebrick
\definecolor{myLGray}{RGB}{225,225,225} % light light gray
%
\newcommand{\todo}[1]{{\color{red}{#1}}}
\newcommand{\blue}[1]{{\color{blue}{#1}}}
\newcommand{\missing}[1]{{\color{blue}{#1}}}
\newcommand{\old}[1]{{\color{lightgray}{#1}}}
\newcommand{\del}[1]{{\color{gray}{#1}}}
\newcommand{\reg}[1]{{\color{myRed2}{#1}}}

\DeclareMathOperator{\argmin}{argmin}
\DeclareMathOperator{\sspan}{span}
\DeclareMathOperator{\res}{Res}
\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\wint}{int}
\DeclareMathOperator{\diam}{diam}
\DeclareMathOperator{\ddiv}{div}
\DeclareMathOperator{\curl}{curl}
\DeclareMathOperator{\ddev}{dev}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\dif}{d}
\DeclareMathOperator{\Dif}{D}
\DeclareMathOperator{\con}{consis}
\DeclareMathOperator{\sym}{sym}
\DeclareMathOperator{\rot}{rot}
\DeclareMathOperator{\hot}{\mbox{h.o.t.}}
\DeclareMathOperator{\Curl}{curl}
\DeclareMathOperator{\Kern}{ker}
\DeclareMathOperator{\rint}{int}
\DeclareMathOperator{\Riesz}{Riesz}
\DeclareMathOperator{\trace}{trace}
\DeclareMathOperator{\dev}{dev}
\DeclareMathOperator{\card}{card}
\DeclareMathOperator{\osc}{osc}
\DeclareMathOperator{\El}{\mathcal{T}}
\DeclareMathOperator{\conv}{conv}
\DeclareMathOperator{\gen}{gen}
\DeclareMathOperator{\midd}{mid}
\DeclareMathOperator{\inn}{int}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\rhs}{rhs}

\newcommand{\dx}{\ensuremath{\, \textrm{d}x }}
\newcommand{\ds}{\ensuremath{\, \textrm{d}s }}
\newcommand{\dt}{\ensuremath{\, \textrm{d}t }}
\newcommand{\deta}{\ensuremath{\, \textrm{d}\eta }}

\newcommand{\deltat}{\ensuremath{\delta_t}}
\newcommand{\deltax}{\ensuremath{\delta_x}}

\newcommand{\px}{\ensuremath{\partial_x}}
\newcommand{\ddt}[1][]{\ensuremath{\tfrac{\text{d}^{#1}}{\text{d}t^{#1}}}}

%% Temporal Discretization

% 'stationary' solution
\def\pb{\xoverline[0.7]{p}}
\def\mb{\xoverline[0.65]{m}}
\def\lb{\xoverline[0.7]{\lambda}}
% difference of p and \pb...
\def\pt{{\widetilde p}}
\def\mt{{\widetilde m}}
\def\lt{{\widetilde \lambda}}
% difference of p0 and \pb...
\def\pot{{\widetilde p}_0}
\def\mot{{\widetilde m}_0}
\def\lot{{\widetilde \lambda}_0}

% Butcher tableau
\newcommand{\fA}{\mathbf{A}}
\newcommand{\fa}{\mathbf{a}}
\newcommand{\fb}{\mathbf{b}}
\newcommand{\fB}{\mathbf{B}}
\newcommand{\fc}{\mathbf{c}}
\newcommand{\fG}{\mathbf{G}}
\newcommand{\fM}{\mathbf{M}}
\newcommand{\fY}{\mathbf{Y}}
\newcommand{\fH}{\mathbf{H}}
\newcommand{\ones}{\mathbbm{1}_s} 

\def\Dt{D_{\tau}}
\def\pn{p_{0,n}}
\def\mn{m_{0,n}}
\def\ln{\lambda_{0,n}}
\def\mun{\mu_{0,n}}
\newcommand{\pj}[1][0]{p_{#1,j}}
\newcommand{\pjm}[1][0]{p_{#1,j-1}}
\newcommand{\pjt}[1][0]{{\widetilde p}_{#1,j}}
\newcommand{\pjmt}[1][0]{{\widetilde p}_{#1,j-1}}
\newcommand{\pkt}[1][0]{{\widetilde p}_{#1,k}}
\newcommand{\mj}[1][0]{m_{#1,j}}
\newcommand{\lj}[1][0]{\lambda_{#1,j}}
\newcommand{\muj}[1][0]{\mu_{#1,j}}

\newcommand{\ps}{\bm{p}}
\newcommand{\pst}{\bm{\widetilde{p}}}
\newcommand{\psj}[1][0]{\bm{p}_{#1,j}}
\newcommand{\psk}[1][0]{\bm{p}_{#1,k}}
\newcommand{\psjt}[1][0]{\bm{\widetilde{p}}_{#1,j}}
\newcommand{\pskt}[1][0]{\bm{\widetilde{p}}_{#1,k}}
\newcommand{\msj}[1][0]{\bm{m}_{#1,j}}
\newcommand{\lsj}[1][0]{\bm{\lambda}_{#1,j}}
\newcommand{\musj}[1][0]{\bm{\mu}_{#1,j}}
\newcommand{\fs}{\bm{\f}}
\newcommand{\gs}{\bm{\g}}
\newcommand{\rs}{\bm{\r}}
\newcommand{\hs}{\bm{\h}}

\newcommand{\nOrd}{\mathsf{n}}
\newcommand{\pOrd}{\mathsf{p}}
\newcommand{\qOrd}{\mathsf{q}}
